Enhancing Item Tokenization for Generative Recommendation through Self-Improvement

Generative recommendation systems, driven by large language models (LLMs), present an innovative approach to predicting user preferences by modeling items as token sequences and generating recommendations in a generative manner. A critical challenge in this approach is the effective tokenization of items, ensuring that they are represented in a form compatible with LLMs. Current item tokenization methods include using text descriptions, numerical strings, or sequences of discrete tokens. While text-based representations integrate seamlessly with LLM tokenization, they are often too lengthy, leading to inefficiencies and complicating accurate generation. Numerical strings, while concise, lack semantic depth and fail to capture meaningful item relationships. Tokenizing items as sequences of newly defined tokens has gained traction, but it often requires external models or algorithms for token assignment. These external processes may not align with the LLM's internal pretrained tokenization schema, leading to inconsistencies and reduced model performance. To address these limitations, we propose a self-improving item tokenization method that allows the LLM to refine its own item tokenizations during training process. Our approach starts with item tokenizations generated by any external model and periodically adjusts these tokenizations based on the LLM's learned patterns. Such alignment process ensures consistency between the tokenization and the LLM's internal understanding of the items, leading to more accurate recommendations. Furthermore, our method is simple to implement and can be integrated as a plug-and-play enhancement into existing generative recommendation systems. Experimental results on multiple datasets and using various initial tokenization strategies demonstrate the effectiveness of our method, with an average improvement of 8\% in recommendation performance.

==> sec/method_bk.tex <==


\section{Method}

Here, we outline the pipeline of our framework, \textbf{SIIT}, which consists of four primary components: item identifier initialization, fine-tuning LLMs for sequential recommendation, item-identifier alignment training, and refining item identifiers using LLMs. Each component will be discussed in detail in the subsequent subsections.


\subsection{Notations}

To begin, we introduce the notations used throughout the paper.  We use $\mathcal{U}$ and $\mathcal{I}$ to represent the sets of all users and items, where $u \in \mathcal{U}$ and $i \in \mathcal{I}$ denote a specific user and item, respectively. Each user $u$ has an interaction sequence $S_u = [i_1, i_2, \dots, i_k]$, and each item $i$ is associated with a semantic feature $C_i$. To integrate with LLMs, each item $i$ can be represented by an identifier that is tokenized into one or more tokens, denoted as $T_i = [t_1, t_2, \dots, t_n]$. These tokens act as unique identifiers within the LLM, and the tokenization of all items is collectively represented by $\mathcal{T}$.

\noindent\textbf{Problem Definition.} Our goal is to perform sequential recommendation using LLMs. Specifically, given a user's interaction history up to timestep $k$, $S_u = [i_1, i_2, \dots, i_k]$, we aim to predict the next item the user will interact with, denoted as $i_{k+1}$.


\subsection{Item Identifier Initialization}\label{sec:init}
In the initial phase of the SIIT framework, we utilize various off-the-shelf item tokenization methods that employ multiple tokens as item identifiers for item identifier initialization. \tz{prob not call SIIT a framework here? maybe sth like: ``prior of siit being used in the gen recsys framework, we can utilize any existing off-the-self ...''} Here, we briefly introduce two popular approaches used during our experimentation: the RQ-VAE-based \tz{let's be consistent on RQVAE or RQ-VAE} method and the hierarchical clustering-based method. Both serve as effective initialization techniques within our framework.

\noindent\textbf{RQVAE-based Tokenization Initialization.} Given an item $i$ with its associated semantic feature $C_i$, RQVAE-based methods first obtain a semantic embedding $x_i$ using a pre-trained semantic extractor (e.g., BERT). This embedding is then compressed into a latent representation $z_i = \text{Encoder}(x_i)$ through an encoder. The latent representation $z_i$ is further quantized into a sequence of codes using a residual vector quantization process over $L$ levels, where $L$ denotes the code length. Specifically, at each quantization level $l$, a learnable codebook $E_l = \{e_k^l\}_{k=1}^N$ is used, where $e_k^l$ represents the $k$-th  codeword embedding at level $l$. The residual quantization process at level $l$ is defined as:

\begin{equation} 
t_l = \arg\min_{k} ||r_l - e_k^l||_2^2 
\end{equation} 
\begin{equation} 
r_{l+1} = r_{l} - e_{t_l} 
\end{equation}

Here, $t_l$ represents the codeword selected at level $l$, and the residual embedding is initialized as $r_1 = z_i$. After $L$ levels of quantization, the item $i$ is represented by a sequence of codewords $T_i = [t_1, t_2, \dots, t_L]$. 

The RQVAE model is typically trained using  reconstruction loss and commitment loss. The reconstruction loss ensures that the quantized latent representation, $\hat{z}_i = \sum_{l=1}^L e_{t_l}$, can recover as much information as possible from the original semantic embedding, and is defined as $\mathcal{L}_{Recon} = ||x_i - \text{Decoder}(\hat{z}_i)||^2$. The commitment loss enforces consistency between the residual and the corresponding codebook embeddings, expressed as $\mathcal{L}_{commit} = \sum_{l=1}^L \left(||\text{sg}(r_l) - e_{t_l}^l||^2 + ||r_l - \text{sg}(e_{t_l}^l)||^2\right)$, where $\text{sg}(\cdot)$ denotes the stop-gradient operation. Additionally, some methods incorporate collaborative regularization and diversity regularization to introduce collaborative signals into the quantized codewords and enhance the diversity of codeword assignments. Further details  can be found in Appendix~\ref{app:RQVAE}.


\noindent\textbf{Hierarchical Clustering Tokenization Initialization.} Another approach to initialize our tokenization is through hierarchical clustering based on item collaborative information (i.e., CID~\cite{cid}).  CID constructs a co-occurrence matrix $O \in \mathbb{R}^{|\mathcal{I}|\times|\mathcal{I}|}$, where each entry indicates the frequency of co-occurrence between two items in a user's interaction sequence. Spectral clustering is then performed on the co-occurrence matrix $O$. If a cluster's size exceeds a predefined threshold, the clustering process is recursively applied within that cluster, yielding hierarchical clusters at increasingly finer levels, as depicted in Figure ~\ref{fig:main}. Items are tokenized according to their respective cluster center at each level, i.e., $T_i = [t_1, t_2, \dots, t_L]$, where $t_l$ denotes the cluster index at level $l$. This method encourages items with higher co-occurrence similarity to share more tokens.


\subsection{Sequential Recommendation Task Training}\label{sec:seq}

Following the item tokenization initialization stage, each item $i$ is represented as an identifier: $T_i = [t_1, t_2, \dots, t_L]$. To fine-tune the LLM backbone, we employ a sequential item prediction task. This involves constructing personalized recommendation prompts that incorporate the user’s historical interactions. The LLM is then tasked with predicting the next item the target user is likely to interact with, based on these instructions and the interaction history. An example prompt is shown below:


\begin{tcolorbox}[colframe=black!75!white, title=Seqential Recommendation Task]
\textbf{Instruction:} This person has bought \texttt{<a\_1> <b\_3> <c\_5> <d\_2>, ... ,<a\_2> <b\_1> <c\_5> <d\_3>} in the previous. Please predict the next product this person will buy. Answer: \\
\textbf{Response:} <a\_1> <b\_2> <c\_7> <d\_1>
\end{tcolorbox}

In our experiments, we utilize 15 templates to generate these prompts (see Appendix~\ref{app:prompt} for details). During training, the model is optimized using a next-token prediction loss applied to the generated responses. Specifically, given the instruction prompt, which includes the user’s interaction history, the objective is to generate the correct next item sequence $T_i = [t_1, t_2, \dots, t_L]$. The loss is calculated as follows:

\begin{equation}
    \mathcal{L} = -\sum_{l=1}^L \text{log } P(t_l|\text{prompt}, t_{< l})
\end{equation}




\tz{secs 2.1-2.3 feel more like preliminary section to me, as they are really just introducing existing things and discribing how genir works right? maybe we can separate sec2 into two sections and break around here, where the method section then concentrates more on what our method adds/differents from the existing framework}

\subsection{Item-Identifier Alignment }\label{sec:align}


After a certain amount of fine-tuning on sequential recommendation tasks, we obtain the model $\mathcal{M}$. At this stage, the model has developed an understanding of the collaborative relationships between items and has integrated this knowledge into the current token embeddings.  We then periodically introduce the Item-Identifier Alignment training to establish a correspondence between the tokenized item $T_i = [t_1, t_2, \dots, t_L]$ and its original semantic feature $C_i$. This correspondence is then used to regenerate and refine the item tokenization. The Item-Identifier Alignment task consists of two subtasks: Item to Identifier and Identifier to Item. \tz{prob Item-to-Identifier and Identifier-to-Item?}

In the Item to Identifier task, we construct an instruction that includes the text feature of the item and prompt the model to generate the corresponding identifier. The prompt format is as follows:

\begin{tcolorbox}[colframe=black!75!white, title=Item to Identifier Task]
\textbf{Instruction:} Please generate the index for the item called \textit{NYX Super Fat Eye Marker,SFEM01 Carbon Black}:  \\
\textbf{Response:} <a\_4> <b\_1> <c\_2> <d\_3>
\end{tcolorbox}

In the Identifier to Item task, the instruction consists of the item identifier, and the model is expected to reconstruct the original semantic feature. The goal is to ensure that the current token embeddings of item identifier preserve the semantic feature to the greatest extent. The prompt format for this task is as follows:

\begin{tcolorbox}[colframe=black!75!white, title=Identifier to Item Task]
\textbf{Instruction:} Please generate the name for the item corresponding to \textit{<a\_4> <b\_1> <c\_2> <d\_3>}: \\
\textbf{Response:} NYX Super Fat Eye Marker,SFEM01 Carbon Black.
\end{tcolorbox}

For both tasks, we also apply the next token prediction loss on the model’s responses during training. After completing the training, we obtain an updated model, $\mathcal{M'}$, which will be used in the subsequent item identifier refinement process.

\subsection{Item Identifier Refinement} \label{sec:generate}

% \runjin{better add figure on the perplexity distrubution}

% \runjin {try to unify name, here I used id}

After obtaining the updated model $\mathcal{M'}$, we observed that while most items achieved a good alignment between their identifier and the corresponding item feature, a few item prompts remained challenging to optimize, consistently showing relatively high perplexity. This indicates that the current tokenization for these items does not fully match the model’s understanding. To address this, we aim to refine the tokenization for such items based on the model’s current state. Specifically, we perform token generation for each item using the item-to-identifier task on $\mathcal{M'}$. The output reflects the identifier that the model currently finds most well-aligned with the item. 
However, this process may lead to identifier collision among similar items. While this is not inherently negative—since the model assigns similar identifiers to items it perceives as similar—it becomes problematic if two items share an identical identifier (ID collision). In such cases, the model cannot differentiate between them, resulting in both items always being recommended simultaneously whenever this identifier is predicted. Through our experiments (Section~\ref{sec: ablation}), we found that this scenario can negatively impact recommendation performance. To mitigate this, we propose a Diverse Token Generation Strategy and a Collision Avoidance Strategy to reduce and eliminate collisions, ensuring that similar items receive different but closely related identifiers, preserving their similarity without resulting in identical identifiers. \tz{let's not use so many ``this'' in one paragraph with them all pointing to different things}

% \runjin{why avoid collid, it's our hope}
\noindent\textbf{Diverse Identifier Generation Strategy.} To prevent item ID collisions, we use beam search instead of greedy search for generating item identifiers. For each item, beam search selects the top $k$ candidate identifiers (with $k=20$ in our experiments) that the model considers most appropriate. We then iterate through the items, checking their ranked list of generated identifiers from front to back. If an identifier has not been assigned to a previous item, it is allocated to the current item. If the identifier is already taken, we move on to the next one in the list. In the rare case where no available identifier remains after scanning the entire ranking list (an occurrence in less than 5\% of cases in our experiments), we temporarily assign the top-ranked identifier and later apply the collision avoidance strategy on them.

\noindent\textbf{Collision Avoidance Strategy.} After completing identifier reassignments for all items, there may still be rare cases where items share the same identifier due to semantic similarities in the model’s current understanding. In such cases, we append a new token to these identifiers to distinguish these items.

At this stage, each item will be assigned a newly refined, unique identifier. We then use these updated item identifiers  to continue sequential recommendation training on the previously fine-tuned model $\mathcal{M}$, which was already trained on the sequential recommendation task. After training for a few more epochs, we have the option to start the next iteration by revisiting the Item-Identifier Alignment and Item Identifier Refinement steps to further refine the tokenization.


\subsection{Inference}

After obtaining the final iteration of item identifiers and finetuned  model, we use this model and identifiers for inference. For each user in the test set, we randomly select one from 15 pre-designed sequential recommendation task prompt templates and construct an instruction based on the current user's history, which is then fed into the model. Since we need to provide a ranking list of potential next items, we apply beam search for output generation. To prevent the model from generating invalid items that are not present in the item set, we utilize constrained beam search. This is achieved by constructing a prefix tree based on all item identifiers, which constrains the output candidates at each step to only valid tokens from the prefix tree according to the current output. Finally, all outputs are ranked by their perplexity score.


% In summary, we present the SIIT framework in Algorithm~\ref{alg
% }. The process begins by initializing the large language model (LLM) with a pretrained model, denoted as $\mathcal{M}_{\text{init}}$, and initializing the item tokenization using an off-the-shelf technique, referred to as $\mathcal{T}0$. The model is then fine-tuned on the sequential recommendation task using $\mathcal{T}0$, resulting in the updated model $\mathcal{M}0$. The iterative self-improving process begins, where for each iteration $i$, the model $\mathcal{M}{i-1}$ is fine-tuned on a text-item alignment task using the tokenization from the previous iteration, $\mathcal{T}{i-1}$. This produces an intermediate model, $\mathcal{M}{i-1}'$, which is then used to generate an improved item tokenization, $\mathcal{T}i$. The model $\mathcal{M}{i-1}$ is subsequently fine-tuned on the sequential recommendation task using $\mathcal{T}_i$, yielding the updated model $\mathcal{M}_i$. This process continues for $n$ iterations. The final output consists of the fine-tuned model $\mathcal{M}_n$ and the refined item tokenization $\mathcal{T}_n$.


In summary, we present the SIIT framework in Algorithm~\ref{alg:siit}. The process begins with a pretrained LLM and an off-the-shelf item tokenization method to initialize item identifiers. The model is initially fine-tuned on a sequential recommendation task using these initial identifiers. Over several iterations, the model alternates between fine-tuning on item-identifier alignment tasks, generating and refining identifiers, and fine-tuning on the recommendation task. Finally, the fully fine-tuned model and the refined identifiers are used for inference.

\begin{algorithm}[H]
    \caption{SIIT: Self-Improving Method for Item Tokenization}
    \label{alg:siit}
    \begin{algorithmic}[1]
        \REQUIRE Number of iterations $n$
        \STATE \textbf{Initialize} the LLM with pretrained model as $\mathcal{M}_{\text{init}}$
        \STATE \textbf{Initialize} item identifiers using an off-the-shelf technique as $\mathcal{T}_0$
        \STATE \textbf{Fine-tune} the model $\mathcal{M}_{\text{init}}$ on the sequential recommendation task using $\mathcal{T}_0$, yielding the updated model $\mathcal{M}_0$
        \FOR{$i = 1$ to $n$}
            \STATE \textbf{Fine-tune} the model $\mathcal{M}_{i-1}$ on the item-identifier alignment tasks using $\mathcal{T}_{i-1}$, yielding $\mathcal{M}_{i-1}'$
            \STATE \textbf{Generate} new item identifiers $\mathcal{T}_i$ using the updated model $\mathcal{M}_{i-1}'$
            \STATE \textbf{Fine-tune} the model $\mathcal{M}_{i-1}$ on the sequential recommendation task using $\mathcal{T}_i$, yielding the updated model $\mathcal{M}_i$
        \ENDFOR
        \STATE \textbf{Perform inference} on the test set using the fine-tuned model $\mathcal{M}_n$ and item identifiers $\mathcal{T}_n$ 
    \end{algorithmic}
\end{algorithm}

